Understanding and Evaluating Racial Biases in Image Captioning

Image captioning is an important task for benchmarking visual reasoning and for enabling accessibility for people with vision impairments. However, as in many machine learning settings, social biases can influence image captioning in undesirable ways. In this work, we study bias propagation pathways within image captioning, focusing specifically on the COCO dataset. Prior work has analyzed gender bias in captions using automatically-derived gender labels; here we examine racial and intersectional biases using manual annotations. Our first contribution is in annotating the perceived gender and skin color of 28,315 of the depicted people after obtaining IRB approval. Using these annotations, we compare racial biases present in both manual and automatically-generated image captions. We demonstrate differences in caption performance, sentiment, and word choice between images of lighter versus darker-skinned people. Further, we find the magnitude of these differences to be greater in modern captioning systems compared to older ones, thus leading to concerns that without proper consideration and mitigation these differences will only become increasingly prevalent. Code and data is available at https://princetonvisualai.github.io/imagecaptioning-bias .

==> Input_Files/Mitigation.tex <==
Based on our analyses, we propose directions for mitigating the biases found in captioning systems. First, from our findings in Sec.~\ref{sec:gender_annot} and~\ref{sec:experiments_racialterms}, we see that human annotators make assumptions about the demographics of people pictured or use different language when describing people of different skin tone groups. To mitigate this, dataset collectors can provide more explicit instructions for annotators (e.g. do not label gender or include racial descriptors to people). In addition, we also find that ground-truth captions contain profane language (Sec.~\ref{sec:experiments_racialterms}). In line with existing mitigation efforts~\cite{yang2020fair, prabhu2020large}, manual captions containing slurs or other offensive concepts should be removed from the dataset. Additionally, in Fig.~\ref{fig:amt_res} we see that only $7.0\%$ of the dataset contained images of people with darker skin tones, i.e., 1096 images. We need to collect more diverse datasets such that we can measure disaggregated statistics and compare metrics such as the difference in SPICE scores with the knowledge that our measurements do not suffer from a high sampling bias. Finally, from our analysis of generated captions (Sec.~\ref{sec:experiments_normalized}), we note that \textbf{Oscar} exhibits less bias compared to the other transformer-based models. This suggests the greater dataset diversity from pre-training the model may help reduce the amount of bias that propagates into the automated captions.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
